Learning-to-Learn Personalised Human Activity Recognition Models

Human Activity Recognition~(HAR) is the classification of human movement, captured using one or more sensors either as wearables or embedded in the environment~(e.g. depth cameras, pressure mats). State-of-the-art methods of HAR rely on having access to a considerable amount of labelled data to train deep architectures with many train-able parameters. This becomes prohibitive when tasked with creating models that are sensitive to personal nuances in human movement, explicitly present when performing exercises. In addition, it is not possible to collect training data to cover all possible subjects in the target population. Accordingly, learning personalised models with few data remains an interesting challenge for HAR research. We present a meta-learning methodology for learning to learn personalised HAR models for HAR; with the expectation that the end-user need only provides a few labelled data but can benefit from the rapid adaptation of a generic meta-model. We introduce two algorithms, Personalised MAML and Personalised Relation Networks inspired by existing Meta-Learning algorithms but optimised for learning HAR models that are adaptable to any person in health and well-being applications. A comparative study shows significant performance improvements against the state-of-the-art Deep Learning algorithms and the Few-shot Meta-Learning algorithms in multiple HAR domains.

==> exploremaml.tex <==
\section{Personalised MAML: Exploratory Study}
\label{sec:explorepmaml}
We perform three exploratory studies to further investigate Personalised MAML~($MAML^p$) with the 4 datasets from \mex for Exercise Recognition. We select \mex datasets because they contain a combination of heterogeneous modalities and are the datasets with least amount of data for a person-class which is the closest representation of a Few-shot Learning setting. 

%maml vs. personalised maml validation accuracy over training epochs

We first investigate the performance improvements achieved by $MAML^p$ after using the Personalised Meta-Learning methodology against $MAML$. 
Accordingly we compare three algorithms, $MAML$ where meta-train and test tasks are created disregard of any person identifiers; $MAML^p$, as described in Section~\ref{sec:pmaml}; and Person-aware $MAML$. 
Here Person-aware $MAML$ can be seen as a lazy personalisation of MAML where a meta-train task is comprised of data instances selected from a set of persons. The support set contains $K^s$ data instances for each activity class, obtained from a single person, not strictly similar to the person selected to provide the query set. 
This method still preserve the concept of ``person-activity'' as the class label, but not constrained to one person. 
We visualise how a meta-model test when trained with these different algorithms in both $K^s=1$ and $K^s=5$ settings using the \mexpm dataset.
we plot test-person accuracy evaluated at every 10 meta-train epochs; at each stop, meta-test support set trains the meta-model for 10 meta-gradient steps, and is evaluated at each meta-gradient step.

\begin{figure}[ht]
\centering
\begin{subfigure}{.5\textwidth}
\centering
\includegraphics[width=0.95\linewidth]{maml-1-shot-3-types}
\caption{$K^s = 1$}
\label{fig:maml_vs_mamlp_1shot}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
\centering
\includegraphics[width=.95\linewidth]{maml-5-shot-3-types}
\caption{$K^s = 5$}
\label{fig:maml_vs_mamlp_5shot}
\end{subfigure}
\caption{MAML vs. Person-aware MAML vs. MAML$^p$ with \mexpm}
\label{fig:maml_vs_mamlp}
\end{figure}

Figures~\ref{fig:maml_vs_mamlp_1shot} and~\ref{fig:maml_vs_mamlp_5shot} compare $MAML$, $MAML^p$ and Person-aware $MAML$ using \mexpm in $K^s=1$ and $K^s=5$ settings respectively.
$MAML^p$ and Person-aware $MAML$ significantly outperformed $MAML$ in both settings. When comparing $MAML^p$ and Person-aware $MAML$, $MAML^p$ algorithm achieves a more generalised meta-model even with zero meta-model adaptation; this is most significant in the $K^s=1$ setting. 
These observations verify the advantage of creating personalised tasks. Even with the Person-aware $MAML$ algorithm, where each task contains data from multiple people, but each ``person-activity'' class only contains data from one person. 
Accordingly, personalised algorithms ensure that the task-models are trained for a set of ``person-activity'' classes instead of ``activity'' classes. 
$MAML^p$ further ensure all ``person-activity'' belong to the same person, allowing further generalisation. 
Another indication of the significance of personalisation is found when investigating $MAML$ performance over the training epochs. While $MAML$ improve overall performance as the meta-model train, $MAML$ meta-test accuracy before adaptation~(every $0^{th}$ meta-gradient step), declines consistently. This is most significant when $K^s=5$, which indicates that the meta-model learned with $MAML$ is not generalised when an activity class in a meta-train task support set contains data from multiple people. In comparison, meta-model learned with $MAML^p$, performs well on meta-test tasks, even before adaptation. 


%query size comparison

Next we explore the most effective $K^q$ value for training $MAML^p$. 
Original $MAML$ experiments used $K^q=K^s$ for image classification~\cite{finn2017model}.
As shown in Algorithm~\ref{algo:pmaml_train} line 8, $K^q$ determine how many data instances are considered in meta-update loss calculation, that later affect meta-model learning. 
Given each meta-train task for $MAML^p$, now belong to a specific person, we expect to find the effect of using a different number of data instance in meta-update.
Accordingly we explore three $K^q$ values 5, 10 and $K-K^s$ where the $K$ is all available data instances for an ``person-activity'' class~(30 on average for all \mex datasets)

\begin{table}[ht]
\caption{MAML$^p$: Exploring meta-train task query set size $K^q$}
\label{tbl:maml_kq}
\centering
\begin{tabular} {@{\hspace{5pt}} l @{\hspace{5pt}} l @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}}}
\toprule
$K^s$&$K^q$&\mexact&\mexacw&\mexdc&\mexpm\\
\midrule
\multirow{3}{*}{1}&5&0.8332&0.5652&0.8230&0.7752\\
&10&0.8414&0.5790&0.8253&0.7834\\
&$K-K^s=29$&0.8431&0.5937&0.8339&0.7912\\
\midrule
\multirow{3}{*}{5}&5&0.9097&0.6701&0.9736&0.9367\\
&10&0.9098&0.6812&0.9778&0.9376\\
&$K-K^s=25$&0.9103&0.6825&0.9774&0.9377\\
\bottomrule
\end{tabular}
\end{table}

Table~\ref{tbl:maml_kq} present results for different $K^q$ values in two settings $K^s=1$ and $K^s=5$ for 4 datasets derived from \mex. 
Both settings achieve comparably similar performances with all $K^q$ values. This suggests that meta-update is not affected adversely by creating personalised tasks, where the meta-update uses loss from person-specific task models. 
We plot the meta-test performance during the 10 gradient steps of meta-model adaptation to visualise the effect of learning a meta-model from different $K^q$ values in Figure~\ref{fig:maml_kq} (Here $K^s$ is set to 5). While both \mexact and \mexpm achieve similar performances with all three meta-models after adaptation, but the most generalised meta-model is learned when using $K^q=5$, as it achieves best performance before and during model adaptation. 
This suggests limiting $K^q$ improve generalisation of the meta-model for later adaptation with a person not seen during training. 

\begin{figure}[ht]
\centering
\begin{subfigure}{.5\textwidth}
\centering
\includegraphics[width=.75\linewidth]{maml-pm-kq}
\caption{PM}
\label{fig:maml_kq_pm}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
\centering
\includegraphics[width=.75\linewidth]{maml-act-kq}
\caption{ACT}
\label{fig:maml_kq_act}
\end{subfigure}
\caption{MAML$^p$: Meta-test task gradient steps on a meta-model trained with $K^q$ }
\label{fig:maml_kq}
\end{figure}


%support set size comparison
Finally we perform an exploratory study of $K^s$ using a range of $K^s$ values. Finding the the balance between $K^s$ and performance of $MAML^p$ is important because, at deployment, the test-person is expected to provide $K^s$ amount of data instances per activity class, therefore its is desirable to keep $K^s$ to a required minimum. We perform experiments with all 4 datasets from \mex for $K^s$ values 1, 3, 5, 7 and 10. 

\begin{comment}
\begin{table}[ht]
\row{1.2}
\caption{MAML$^p$: Exploring meta-training $K^s$}
\label{tbl:maml_ks}
\centering
\begin{tabular} {@{\hspace{5pt}} l @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r  @{\hspace{5pt}}}
\toprule
\multirow{2}{*}{Dataset}&\multicolumn{6}{c}{$K^s$}\\
\cline{2-7}
&1&3&5&7&10&13\\
\hline
\mexact&0.8431&0.8991&0.9103&0.9204&0.9237&0.9170\\
\mexacw&0.5937&0.6753&0.6825&0.6917&0.6944&0.6910\\
\mexdc&0.8339&0.9537&0.9774&0.9863&0.9921&0.9938\\
\mexpm&0.7912&0.9098&0.9377&0.9494&0.9564&0.9593\\
\bottomrule
\end{tabular}
\end{table}
\end{comment}

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
\centering
\includegraphics[width=.75\linewidth]{maml-ks-mex}
\caption{$K^s$}
\label{fig:maml_kshot}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
\centering
\includegraphics[width=.75\linewidth]{maml-pm-kshot-test}
\caption{ACT}
\label{fig:maml_act_kshot_train}
\end{subfigure}
\caption{MAML$^p$: Exploring meta-training $K^s$}
\label{fig:maml_kshot_train}
\end{figure}


Figure~\ref{fig:maml_kshot} plot meta-test performances obtained by datasets \mexact, \mexacw, \mexdc and \mexpm. Increasing $K^s$ consistently improve performance up to $K^s=10$ and report decreased or similar performance  when $K^s=13$ with all datasets.
A significant performance improvement is observed when increasing $K^s$ from 1 to 3. While modalities ACT and ACW achieve highest performance with $K^s=10$ modalities DC and PM gradually improve performance even at $K^s=13$. The visualisation of test accuracy at every 10 epochs during training further verify improved performance with increasing $K^s$. 



==> explorern.tex <==
\section{Personalised RN: Exploratory Study}
\label{sec:exploreprn}

We perform two exploratory studies to further investigate Personalised Relation Network~($RN^p$). Again we use the four datasets from \mex for this study. 

First we compare the performance between the two algorithms Relation Networks~(RN) and $RN^p$ to understand the effect of personalisation on network training and testing. 
For this purpose we train the two algorithms, with the \mexpm dataset in two setting $K^s=1$ and $K^s=5$ for 300 epochs, and evaluate each model at every 5 epochs.

\begin{figure}[ht]
\centering
\begin{subfigure}{.5\textwidth}
\centering
\includegraphics[width=.8\linewidth]{rn-pvsnp-1shot}
\caption{1-shot}
\label{fig:rn_pvsnp_1shot}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
\centering
\includegraphics[width=.8\linewidth]{rn-pvsnp-5shot}
\caption{5-shot}
\label{fig:rn_pvsnp_5shot}
\end{subfigure}
\caption{RN vs. RN$^p$ with \mexpm meta-model tested at every 10 meta-train epochs}
\label{fig:rn_pvsnp}
\end{figure}

In Figures~\ref{fig:rn_pvsnp_1shot} and~\ref{fig:rn_pvsnp_5shot} plot the two algorithms RN and $RN^p$ accuracy on meta-test tasks for the two settings $K^s=1$ and $K^s=5$. 
It is evident that personalisation has a stabilised the meta-training process, where meta-test models perform consistently with $RN^p$ models. 
In contrast meta-test evaluation on the $RN$ models is erratic, that is especially significant when $K^s=5$. When training $RN$ in the $K^s=5$ setting, a task is created disregard of the person parameter, as a result, a class contains data instances from more than one person and learning similarities to many people has adversely affected the learning of the $RN$ meta-model. Similarly, in the $K^s=1$ setting, when a task contains only one data instance per class, learning from yourself~($RN^p$) is found more advantages.

%support set size comparison

Next we explore different $K^s$ values to find the most optimal value; similar to $MAML^p$, $K^s$ determine how many data instances are required from a new person for the optimal personalisation of the model; therefore, we try to find the balance between performance improvement and $K^s$. Accordingly we create 10 experiments with each \mex dataset; \mex datasets give us the opportunity to compare how modalities recorded for the same set of activities with different placements respond to having few or many support set data for comparison at test time.

\begin{comment}
\begin{table}[ht]
\row{1.2}
\caption{RN: Exploratory Study}
\label{tbl:rn_spt_size}
\centering
\begin{tabular} {@{\hspace{5pt}} l @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}}}
\toprule
\multirow{2}{*}{Dataset}&\multicolumn{5}{c}{$K^s$}\\
\cline{2-6}
&1&3&5&7&10\\
\hline
\mexact&0.9322&0.9439&0.9436&0.9464&0.9376\\
\mexacw&0.7783&0.7653&0.7719&0.7687&0.7716\\
\mexdc&0.9147&0.9351&0.9205&0.9161&0.9034\\
\mexpm&0.7816&0.8416&0.8520&0.8574&0.8534\\
\bottomrule
\end{tabular}
\end{table}
\end{comment}

\begin{figure}[ht]
\centering
\includegraphics[width=0.6\textwidth]{rn-kshot-mex}
\caption{RN$^p$ Different $K^s$ with \mexact, \mexacw, \mexdc and \mexpm}
\label{fig:rn_ks}
\end{figure}

We plot averaged accuracy against different $K^s$ for each dataset in Figure~\ref{fig:rn_ks}, which shows that different datasets prefer different $K^s$ values.
Both \mexact and \mexdc exhibit dome shaped behaviour with increasing $K^s$ sizes where after $K^s=7$ it is detrimental to the network to have many examples of the same activity class for comparison. 
In contrast, \mexpm dataset show continuous performance increment with increasing $K^s$ and at $K^s=10$ it starts to dome like other modalities. 
%We are unable to explain the behaviour of \mexacw :) 

As mentioned in Section~\ref{sec:results}, a larger $K^s$ value increases the memory requirements of the algorithm and takes longer to perform a single classification task. An HAR algorithm should be able to recognise activities as they are performed in real-time for the best user-experience, and the response time and processor and memory requirements crucial factors for consideration. 


% different similarity learning modules
\begin{comment}
\begin{table}[ht]
\caption{RN$^p$: Exploring $\theta_r$}
\label{tbl:rn_thetar}
\centering
\begin{tabular} {@{\hspace{5pt}} l @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}}}
\toprule
Algorithm&\mexact&\mexacw&\mexdc&\mexpm\\
\midrule
RN&0.9327&0.7279&0.8189&0.8145\\
$RN^p$&\textbf{0.9436}&\textbf{0.7719}&\textbf{0.9205}&\textbf{0.8520}\\
$RN^p$(cce)&\textbf{0.9453}&0.7623&0.9031&\textbf{0.8533}\\
$RN^p$+ATT(mse)&\textbf{0.9403}&0.7600&0.8910&\textbf{0.8534}\\
$RN^p$+ATT(cce)&\textbf{0.9429}&0.7514&0.8862&0.8466\\
\bottomrule
\end{tabular}
\end{table}
\end{comment}


==> pmamlinference.tex <==
\section{Improved Inference of Personalised MAML}
\label{sec:pmamlinference}

\begin{table}[ht]
\caption{}
\label{tbl:pmamlinference}
\centering
\begin{tabular} {@{\hspace{5pt}} l @{\hspace{5pt}} c @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}}}
\toprule
$K^s$&neighbours&\mexact&\mexacw&\mexdc&\mexpm\\
\midrule
\multirow{4}{*}{1}&0&0.8431&0.5937&0.8339&0.7916\\
&1&\textbf{0.8812}&0.4809&0.77989&\textbf{0.8318}\\
&3&0.8482&0.3892&0.7262&\textbf{0.8189}\\
&5&0.8330&0.3501&0.6825&\textbf{0.8206}\\
\midrule
\multirow{4}{*}{3}&0&0.8991&0.6753&0.9537&0.9098\\
&1&\textbf{0.9098}&0.5320&0.9125&\textbf{0.9227}\\
&3&0.8849&0.4268&0.8579&0.9084\\
&5&0.8739&0.3836&0.8071&0.9045\\
\midrule
\multirow{4}{*}{5}&0&0.9103&0.6825&0.9774&0.9377\\
&1&\textbf{0.9218}&0.5408&0.9479&\textbf{0.9505}\\
&3&0.8946&0.4372&0.8926&0.9362\\
&5&0.8726&0.3930&0.8247&0.9325\\
\bottomrule
\end{tabular}
\end{table}
